Anytime Probabilistically Constrained Provably Convergent Online Belief Space Planning

Taking into account future risk is essential for an autonomously operating robot to find online not only the best but also a safe action to execute. In this paper, we build upon the recently introduced formulation of probabilistic belief-dependent constraints. We present an anytime approach employing the Monte Carlo Tree Search (MCTS) method in continuous domains. Unlike previous approaches, our method assures safety anytime with respect to the currently expanded search tree without relying on the convergence of the search. We prove convergence in probability with an exponential rate of a version of our algorithms and study proposed techniques via extensive simulations. Even with a tiny number of tree queries, the best action found by our approach is much safer than the baseline. Moreover, our approach constantly finds better than the baseline action in terms of objective. This is because we revise the values and statistics maintained in the search tree and remove from them the contribution of the pruned actions.

==> floats/CPFTDPW_tableLightDark.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\textbf{Model}  &SIM. calls & MCTS mode & Rollout  &$\hat{V}^*(b_0; \boldsymbol{\rho}_1)$  & $\hat{\mathrm{P}}(S|b_0)$ &  num. coll\\
\midrule
\texttt{CPFT-DPW}  & $15$ & average & Yes &$-75.67 \pm 57.66$ &    $0.77$    & $16/70$\\
\midrule
{\bf PCPFT-DPW}&   $15$  & average &  Yes &    $ -115.27 \pm 94.28 $ &          $1$             & $0/70$ \\ 
\bottomrule
\end{tabular}}
\caption{Here we study anytime safety, $\tilde{\delta}{=}1{-}\delta {=} 0$ and $500$ belief particles. In the Light Dark problem, the robot performs $5$ steps of alternating planning and execution sessions.  We do $70$ trials of each such  a scenario and approximate the $\mathrm{P}(\{\tau_0 {\in} \times_{\ell=0}^{L}\mathcal{X}^{\mathrm{safe}}_{\ell}|b_0)$, where $\tau_0 {=} x_{0:L}$. The event $S{=}\{\tau_0 {\in} \times_{\ell=0}^{L}\mathcal{X}^{\mathrm{safe}}_{\ell}\}$ means each state in the actual robot trajectory starting at time $0$ was safe. $\hat{V}^*(b_0;\boldsymbol{\rho}) {=} \frac{1}{70}\sum_{i=1}^{70} \sum_{\ell=0}^{4} \rho_{\ell+1}(b^i_{\ell},a^i_{\ell}, b^i_{\ell+1})$ where $\rho_{\ell+1}(b_{\ell},a_{\ell}, b_{\ell+1})$ is defined in \eqref{eq:LDreward}. The rollout of CPFT is a random policy. The rollout of Alg.~\ref{alg:CCPCMCTS} (PCPFT-DPW) is the Alg.~\ref{alg:SafeRollout}, namely our safe rollout.}
\label{tbl:LDprop}
\end{table*}

==> floats/CPFTDPW_tableRoomba.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\textbf{Model}  & tree queries & MCTS mode   &$\hat{V}^*(b_0; \boldsymbol{\rho}_1)$  & $ \hat{\mathbb{E}}[\|x^{t} - x^{g}\|^2_2]\pm \mathrm{std} $ &$ \hat{\mathrm{P}}(S|b_0)$  & num. coll\\
\midrule
\texttt{CPFT-DPW}  & $100$ & average (Fig.~\ref{fig:MCTS})  &$-50000\pm 0 $ &    $1014.57 \pm 421.66$  & $1$ & $0/70$\\
\midrule
{\bf PCPFT-DPW}  &$100$ & $\substack{ {\text{average }} \\ {\text{only safe actions}}}$     &$ -25300 \pm 13335$ &  $98.52 \pm 330.04$   & $0.96$  & $3/70$\\
\midrule
\texttt{CPFT-DPW}  &$1000$ & average (Fig.~\ref{fig:MCTS})  &$-46500.0 \pm 136.31$ &  $829.78 \pm 525.88$     & $1$ &$0/70$\\
\midrule
{\bf PCPFT-DPW}  &$1000$ & $\substack{ {\text{average }} \\ {\text{only safe actions}}}$    &$ -28086 \pm 14399 $ & $56.86 \pm 215.12$    & $1$ & $0/70$\\
\midrule
\texttt{CPFT-DPW}  & $15$ &  average (Fig.~\ref{fig:MCTS})  &$-48728.73 \pm 77.64$ &  $841.28 \pm 484.55$   & $0.97$ & $2/70$\\
\midrule
{\bf PCPFT-DPW}  & $15$ & $\substack{ {\text{average }} \\ {\text{only safe actions}}}$   &$-28671.4\pm 13485.07$ &  $70.82 \pm 236.55$    & $0.986$  & $1/70$\\
\bottomrule
\end{tabular}}
\caption{The Lidar Roomba problem with $500$ belief particles and $\delta {=} 1.0$. The robot performs at most $50$ steps of alternating planning and execution sessions.  We do $70$ trials of each such  a scenario and calculate the $\mathrm{P}(S|b_0)$. The event $S{=}\{\tau_0 {\in} \times_{\ell=0}^{L}\mathcal{X}^{\mathrm{safe}}_{\ell}\}$, where $\tau_0 {=} x_{0:L}$ means each state in the actual robot trajectory starting at time $0$ was safe. $\hat{V}^*(b_0;\boldsymbol{\rho}_1) {=} \frac{1}{70}\sum_{i=1}^{70} \sum_{\ell=0}^{L(i)} \rho_{\ell+1}(b^i_{\ell},b^i_{\ell+1})$. The rollout of CPFT-DPW is constant zero. }
\label{Tbl:depart}
\end{table}
